Quantum self-organization and nuclear collectivities

The quantum self-organization is introduced as one of the major underlying mechanisms of the quantum many-body systems, for instance, atomic nuclei. It is shown that atomic nuclei are not necessarily like simple rigid vases containing almost free nucleons, in contrast to the naive Fermi liquid picture. Nuclear forces are demonstrated to be rich enough to change single-particle energies for each eigenstate, so as to enhance the relevant collective mode. When the quantum self-organization occurs, single-particle energies can be self-organized (or self-optimized), being enhanced by (i) two quantum liquids, e.g., protons and neutrons, (ii) two major force components, e.g., quadrupole interaction (to drive collective mode) and monopole interaction (to control resistance). Type II shell evolution is considered to be a simple visible case involving excitations across a (sub)magic gap. Actual cases such as shape coexistence, quantum phase transition, octupole vibration/deformation, super deformation, etc. can be studied with this scope. The quantum self-organization becomes more important in heavier nuclei where the number of active orbits and the number of active nucleons are larger. With larger numbers of them, the effects of the organization can be more significant. The quantum self-organization is a general phenomenon, and is expected to be found in other quantum systems.

==> iopart-num.tex <==
%% input by TO
@article{mayer1949,
  title = {},
  author = {Mayer, Maria Goeppert},
  journal = {Phys. Rev.},
  volume = {75},
  issue = {},
  pages = {1969},
  numpages = {0},
  year = {1949},
  month = {},
  publisher = {},
}

@article{haxel1949,
  title = {},
  author = {Haxel, Otto and Jensen, J. Hans D. and Suess, Hans E.},
  journal = {Phys. Rev.},
  volume = {75},
  pages = {1766},
  numpages = {0},
  year = {1949},
  month = {},
  publisher = {},
}

@book{mayer_jensen_book,
  author={Mayer, M. G. and Jensen, J. H. D.}, 
  title={Elementary Theory of Nuclear Shell Structure},
  publisher={Wiley},
  address={New York}, 
  year={1955},  
}

@book{talmi_book,
  author={de-Shalit A. and Talmi, I.}, 
  title={Nuclear Shell Theory},
  publisher={Dover},
  address={}, 
  year={2004},  
}

@book{heyde_book,
  author={Heyde, K. L. G.}, 
  title={The Nuclear Shell Model},
  publisher={Springer},
  address={}, 
  year={1990},  
}

@article{rmp_SM,
  author = "E. Caurier and G. Mart\'inez-Pinedo and F. Nowacki and A. Poves and A. P. Zuker",
  journal = "Rev. Mod. Phys.",
  volume = "77",
  pages = "427",
  year = "2005",
}

@article{rainwater1950,
  title = {},
  author = {Rainwater},
  journal = {Phys. Rev.},
  volume = {79},
  pages = {432},
  numpages = {},
  year = {1950},
  month = {},
  publisher = {},
}

@article{bohr1952,
  title = {},
  author = {A. Bohr},
  journal = {Mat. Fys. Medd. Dan. Vid. Selsk.},
  volume = {26},
  issue = {14},
  pages = {},
  numpages = {},
  year = {1952},
  month = {},
  publisher = {},
}

@article{bohr_mottelson1953,
  title = {},
  author = {A. Bohr and B. R. Mottelson},
  journal = {Mat. Fys. Medd. Dan. Vid. Selsk.},
  volume = {27},
  issue = {16},
  pages = {},
  numpages = {},
  year = {1952},
  month = {},
  publisher = {},
}

@book{bohr_mottelson_book2,
  author = "A. Bohr and B. R. Mottelson",
  title = "Nuclear Structure",
  volume = 2,
  volumetitle = "Nuclear Deformations",
  publisher = "Benjamin",
  address = "New York",
  year = "1975"
}

@article{schaefer2014,
  author = "T. Schaefer",
  journal = "Nucl. Phys. A",
  volume = "928",
  pages = "180",
  year = "2014",
}
 
@misc{nudat2,
  author = {NNDC}, 
  title = {NuDat 2},
  howpublished = "\url{http://www.nndc.bnl.gov/nudat2/}", 
  year = {2016}
}

@article{togashi2016,
  author = "T. Togashi and Y. Tsunoda and T. Otsuka and N. Shimizu",
  journal = "Phys. Rev. Lett.",
  volume = "117",
  pages = "172502",
  year = "2016",
}


@article{kremer2016,
  author = "C. Kremer and S. Aslanidou and S. Bassauer and M. Hilcker and A. Krugmann and P. von Neumann-Cosel and T. Otsuka and N. Pietralla and V. Yu. Ponomarev and N. Shimizu and M. Singer and G. Steinhilber and T. Togashi and Y. Tsunoda and V. Werner and M. Zweidinger",
  journal = "Phys. Rev. Lett.",
  volume = "117",
  pages = "172503",
  year = "2016",
}

@article{jahn1937,
  author = "H. A. Jahn and E. Teller",
  journal = "Proc. R. Soc. A",
  volume = "161",
  pages = "220",
  year = "1937",
}

@article{otsuka2005,
  author = "T. Otsuka and T. Suzuki and R. Fujimoto and H. Grawe and Y. Akaishi",
  journal = "Phys. Rev. Lett.",
  volume = "95",
  pages = "232502",
  year = "2005",
}

@article{otsuka2010,
  author = "T. Otsuka and T. Suzuki and M. Honma and Y. Utsuno and N. Tsunoda and K. Tsukiyama and M. Hjorth-Jensen",
  journal = "Phys. Rev. Lett.",
  volume = "104",
  pages = "012501",
  year = "2010",
}

@article{otsuka2016,
  author = "T. Otsuka and Y. Tsunoda",
  journal = "J. Phys. G",
  volume = "43",
  pages = "024009",
  year = "2016",
}

@article{tsunoda2014,
  author = "Y. Tsunoda and T. Otsuka and N. Shimizu and M. Honma and Y. Utsuno",
  journal = "Phys. Rev. C",
  volume = "89",
  pages = "031301(R)",
  year = "2014",
}

@article{leoni2017,
  author = "S. Leoni and B. Fornal and others",
  journal = "Phys. Rev. Lett.",
  volume = "118",
  pages = "162502",
  year = "2017",
}

@article{morales2017,
  author = "A.I. Morales and G Benzoni and others",
  journal = "Phys. Lett. B",
  volume = "765",
  pages = "328",
  year = "2017",
}







